Adaptive Sampling for Minimax Fair Classification

Machine learning models trained on uncurated datasets can often end up adversely affecting inputs belonging to underrepresented groups. To address this issue, we consider the problem of adaptively constructing training sets which allow us to learn classifiers that are fair in a minimax sense. We first propose an adaptive sampling algorithm based on the principle of optimism, and derive theoretical bounds on its performance. We also propose heuristic extensions of this algorithm suitable for application to large scale, practical problems. Next, by deriving algorithm independent lower-bounds for a specific class of problems, we show that the performance achieved by our adaptive scheme cannot be improved in general. We then validate the benefits of adaptively constructing training sets via experiments on synthetic tasks with logistic regression classifiers, as well as on several real-world tasks using convolutional neural networks (CNNs).

==> Discussion.tex <==

%===============================================================================
% REMARK ON THE PARAMETER C
%===============================================================================
% \paragraph{Knowledge of parameter $C$ in \algoref{algo:algo1}.}
% The implementation of \algoref{algo:algo1}, as described in Sec.~\ref{sec:algorithm}, requires the knowledge of the parameter $C$ introduced in \assumpref{assump:ideal_case3}. This is primarily because we used the abstract expressions $\{e_z(N): z \in \mc{Z}, \; N \in \N\}$ in presenting and analyzing the algorithm. However, knowing this parameter is not strictly necessary to achieve the same asymptotic convergence rate as in Theorem~\ref{theorem:regret_simple} and Corollary~\ref{corollary:asymptotic}. For instance if we know some constant $0<\beta<1$ such that $\limsup_{N \to \infty} \max_{z \in \mc{Z}} e_z(N)/N^\beta = 0$, then we can achieve the same asymptotic excess risk rate by replacing $\sqrt{N_{z,t}}$ with $N_{z,t}^{\beta}$  in Line~\ref{algoline:forced1} of \algoref{algo:algo1} and removing the $C$ dependent term from Line~\ref{algoline:choose}. For most commonly used function classes $\mc{F}$, any choice of $\beta>0.5$ should suffice. Further details are in Appendix~\ref{appendix:}. \ssnotes{TODO} 


%===============================================================================
% COMPARISON WITH THE ALB PROBLEM
%===============================================================================


% To make the discussion concrete, consider an ALB problem with two distributions $Q_1 \sim N(\mu_1, \sigma_1^2)$ and $Q_2 \sim N(\mu_2, \sigma_2^2)$ for $\mu_1, \mu_2 \in \reals$ and $\sigma_1^2, \sigma_2^2 \in (0,\infty)$. Let  $N_{i,t}$ denote the number of samples allocated by an agent to $Q_i$ for $i=1,2$ and $t\geq 1$. Then, we can construct high probability confidence sequences around $\hat{\mu}_{i,t}$ (the empirical counterparts to $\mu_i$ at time $t$) of non-increasing~(in $t$) lengths $e_{i,t}$ such that $|\hat{\mu}_{i,t}-\mu_i|\leq e_{i,t}$. If at time $t$, the agent decides to draw a sample from arm $1$, it would not change the quality of its estimate of $Q_2$ at time $t+1$ and beyond.  

% On the other hand, let us  consider Instance~2 of \toymodel$(\Mu)$~(introduced in \defref{def:toymodel}) with $\mc{F}$ being the set of all  linear classifiers passing through origin. This is illustrated in \figref{fig:toy_example1}, where the circles denote the one-square-deviation region around the mean values. The shaded circles correspond to the attribute $Z=b$, and the circles with dashed boundaries correspond to the label $Y=0$. For example, $P_{X|YZ}(\cdot|Y=0,Z=a)$ is denoted by the top left circle.
% Suppose at some time $t_1$, the current classifier $\hat{f}_{t_1}$~(represented by the solid gray line passing through origin in \figref{fig:toy_example1}) has low~(resp. high) accuracy for the protected attribute $Z=b$~(resp. $Z=a$).  To remedy this, the agent may draw more samples from the distribution of attribute $Z=b$ to skew the training dataset distribution towards $Z=b$. This would result in the updated classifier $\hat{f}_{t_2}$~(the dashed gray line in \figref{fig:toy_example1}) at some time $t_2>t_1$ to achieve high accuracy for the attribute $Z=b$. But this increased accuracy for $Z=b$ comes at the cost of a reduction in the prediction accuracy for the attribute $Z=a$, as shown in \figref{fig:toy_example1}. 

% The above discussion highlights the key distinguishing feature of our problem from the prior work in ALB. Because of this distinction, the existing analyses of the ALB algorithms do not carry over directly to our case. As a result, to quantify the performance of \algoref{algo:algo1}, we device a new `multi-phase' approach which is described in  detail in Sec.~\ref{subsec:main_results} and Appendix.~\ref{proof:excess_risk1}.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=3in]{instance2_classifier.png}
%     \caption{Figure demonstrates the second instance of \toymodel~introduced in Sec.~\ref{subsec:motivating_example}. Here the circles denote the one-standard-deviation regions of the distributions of features $X$ conditioned on $Y$ and $Z$. Shaded circles correspond to $Z=a$ and circles with dashed boundaries represent $Y=0$. The solid gray line represents a possible  linear classifier that may be learned if the dataset has fewer examples from $Z=b$. If an adaptive algorithm addresses this by populating the data-set with numerous examples from $Z=b$, a possible updated linear classifier is shown by the dashed gray line. This demonstrates the main distinguishing feature of our problem w.r.t. the active learning in bandits~(ALB) problem: \emph{allocating samples to improve the performance on one attribute can have an adverse effect on the performance of the resulting classifier on other attributes}. \ssnotes{move to appendix}}
%     \label{fig:toy_example1}
% \end{figure}
%_______________________________________________________________________________

%===============================================================================
%===============================================================================
% \paragraph{Extension to Pareto Optimal Minimax Fairness.}
% As we saw in Prop.~\ref{prop:sufficient}, Assumptions~\ref{assump:ideal_case}~and~\ref{assump:ideal_case2} together ensure that there exists a unique $\pi^*$ which equalizes the expected loss for all the attributes. We used this fact in our analysis and obtained bounds on the excess risk of the two strategies. However, in many instances these assumptions may not hold, and in these cases the mixture distribution $\pi^*$ achieving the pareto minimax optimal loss may not be unique. 

%===============================================================================
%===============================================================================
% \paragraph{Extension to other fairness measures.}
% In this paper, we have focused mainly on finding the best mixture distribution for the minimax notion of fairness. As mentioned earlier, however, there exist several other fairness measures which may be more suited to certain problems, and often the learning problem is written as the following constrained optimization problem
% \begin{align}
%      &\underset{f \in \mc{F}}{\text{minimize}}\quad \sum_{z \in \mc{Z}} \pi(z) L(z, f)  \\
%      &\text{subject to} \quad \mbb{E}\lb g_k(f, X, Y) \rb \leq 0, \quad \text{ for } k=1,\ldots, K.
% \end{align}
% By appropriately choosing the functions $g_k$, the $K$ constraints can enforce the requirements of various fairness measures such as \emph{demographic parity} and \emph{equalized odds} as described in \citep[\S~2]{agarwal2018reductions}. 

% The techniques developed in this paper can be used to deal with the above formulation in two ways. First, if we consider the unconstrained version of the above problem of $\min_{f \in \mc{F}} \mc{L}\lp \pi, f, \bm{\lambda} \rp \coloneqq \lp \sum_{z \in\mc{Z}} \pi(z)L(z, f) + \sum_{k=1}^K \lambda_k \mbb{E}\lb g_k(f, X, Y)\rb \rp$ \ssnotes{TODO}




==> TheoreticalResults.tex <==
%===============================================================================
% \subsection{Upper bound on excess risk}
% \label{subsec:upper_simple}
%===============================================================================
% \vspace{-0.5em}
In this section, we derive an upper-bound on the excess risk $\mathcal{R}_n(\Aopt)$ of the optimistic adaptive sampling scheme $\Aopt$ (\algoref{algo:algo1}). We begin by describing the assumptions required for our theoretical analysis in Section~\ref{subsec:assumptions}. Then in Section~\ref{subsec:existence}, we prove that under Assumptions~\ref{assump:ideal_case} and~\ref{assump:ideal_case2}, there exists an \emph{ideal} mixture distribution $\pi^*$ at which the optimal classifier optimizes the loss for all attributes. We present and discuss our bound on the excess of \algoref{algo:algo1} in Section~\ref{subsec:analysis_algo1}. In Section~\ref{subsec:analysis_epsilon_greedy}, we formally introduce the \epsg sampling strategy proposed in~\citet{abernethy2020adaptive} and go beyond their analysis to  obtain a bound on its excess risk using the techniques that we have developed in Section~\ref{subsec:analysis_algo1}.
% ~\citet{abernethy2020adaptive} showed the asymptotic consistency of their \epsg strategy in a one-dimensional class of problems, and also derived a finite sample result for its non-exploratory ($\epsilon=0$) instance. However, they did not obtain the convergence rate of its excess risk. We address this by suitably modifying the technical ideas developed for analyzing our optimistic adaptive sampling strategy ($\Aopt$) to obtain an excess risk bound for their \epsg strategy (Theorem~\ref{theorem:epsilon_greedy}).
Finally, in Section~\ref{subsec:lower_bound}, we show that the performance achieved by the our algorithm cannot in general be improved, by obtaining an algorithm independent lower-bound on the excess risk for a particular class of problems. 

%\vspace{-0.5em}

\subsection{Assumptions}
\label{subsec:assumptions}

% \vspace{-0.5em}
% We now state our assumptions on the set of distributions $\{P_z : z \in \mc{Z} \}$, function class $\mc{F}$, and loss function $\loss$ needed for analysing our proposed adaptive sampling scheme.

% \begin{assumption}
% \label{assump:ideal_case}
% The mapping $\pi \mapsto \mbb{E}_z \lb \loss \lp f_\pi, X, Y\rp \rb$ is continuous for all attributes $z \in \mc{Z}$. Furthermore, if $\pi, \nu \in \Delta_m$ are such that $\pi(z) > \nu(z)$ for an attribute $z\in \mc{Z}$, then $\mbb{E}_z \lb \loss(f_\pi, X, Y) \rb < \mbb{E}_z \lb \loss(f_\nu, X, Y)\rb$.
% \end{assumption}    

% The above assumption indicates that increasing the weight of an attribute $z$ in the mixture distribution must lead to an increase in the performance of the resulting classifier on the distribution $P_z$. This assumption provides a natural framework for studying the effect of the composition of the training set on the resulting fairness properties of the learned classifier, which is our focus in this paper.

% \begin{assumption}
% \label{assump:ideal_case2}
% For any two distinct attributes $z, z' \in \mc{Z}$, we must have $\mbb{E}_z \lb \loss(f^*_z, X, Y)\rb < \mbb{E}_{z'} \lb \loss(f^*_z, X, Y)\rb$, for any $f^*_z \in \argmin_{f \in \mc{F}}\, \mbb{E}_z \lb \loss(f, X, Y)\rb$. 
% \end{assumption} 

% This assumption requires that any optimal classifier corresponding to distribution $P_z$ to have higher loss w.r.t.~the distribution $P_{z'}$ of any other attribute $z'\in\mc{Z}$. While it may not always hold (e.g.,~if one attribute is \emph{significantly} easier to classify than another), this assumption, together with \assumpref{assump:ideal_case}, ensure the existence of an optimal mixture distribution $\pi^*$ that equalizes the performance of $f_{\pi^*}$ over all attributes (see Proposition~\ref{prop:sufficient}). In other words, these two assumptions define a regime where it is possible to achieve complete parity in the classification performance across all attributes, by selecting an appropriate mixture $\pi^*$. 
%  Hence it is a natural setting to study the limits of  an adaptive dataset construction strategy in achieving fair classification performance.

\begin{assumption}
\label{assump:ideal_case3}
There exist positive constants $\epsilon_0, C >0$ such that for any function $f \in \mc{F}$ and any $\pi \in \Delta_m$ with $\pi(z)>0,\;\forall z \in \mc{Z}$, if we have $\mbb{E}_\pi \lb \loss \lp f, X, Y \rp \rb \leq \mbb{E}_\pi \lb \loss \lp f_\pi, X, Y \rp \rb + \epsilon$, for some $0 < \epsilon \leq \epsilon_0$, then $ \pi(z) \times \lvert \mbb{E}_z \lb \loss \lp f, X, Y \rp \rb - \mbb{E}_z \lb \loss \lp f_\pi, X, Y \rp \rb \rvert \leq C \epsilon,\;\forall z \in \mc{Z}$.
\end{assumption}
 
This assumption requires that whenever for a $f$ and a $\pi$, $\sum_{z} \pi(z)\big(\mbb{E}_z \lb \loss(f, X, Y) \rb - \mbb{E}_z \lb \loss(f_\pi, X, Y) \rb\big)$ is small, the \emph{absolute value} of the individual components of the sum, i.e., $\pi(z)\lvert \mbb{E}_z \lb \loss(f, X, Y) \rb - \mbb{E}_z \lb \loss(f_\pi, X, Y) \rb \rvert$, cannot be too large. Note that this does not exclude the chance that $\lvert \mbb{E}_z \lb \loss(f, X, Y) \rb - \mbb{E}_z \lb \loss(f_\pi, X, Y) \rb \rvert$ is large; for instance, when $\pi(z)$ is small for some $z$. A sufficient condition for this assumption to hold is that the mapping  $\pi \mapsto f_{\pi}$ is injective, and any other local optimizer is at least $\epsilon_0$ sub-optimal. 

\begin{assumption}
\label{assump:uniform_deviation}
Let $\delta\in [0,1]$ be a confidence parameter. For each $z\in\mc{Z}$, there exists a monotonically non-increasing sequence $\{ e_{z} \lp N, \mc{F}, \delta \rp : N \geq 1\}$ with $\lim_{N \to \infty} e_{z} \lp N, \mc{F}, \delta \rp = 0$, such that the following event holds with probability at least $1-\delta/2$:

\vspace{-0.25in}
\begin{small}
\begin{align*} 
\Omega = \bigcap_{z \in \mc{Z}} \bigcap_{N=1}^\infty \Big\{\sup_{f \in \mc{F}}\, \big\vert \widehat{L}_N(z, f) - L(z, f) \big\vert \leq e_{z}(N, \mc{F}, \delta)
%  ,  \;\; \forall z \in \mc{Z}, \;  1 \leq N \leq n
\Big\},
\end{align*} 
\end{small}
\vspace{-0.20in}

where $\widehat{L}_N(z, f) \coloneqq \frac{1}{N} \sum_{i=1}^N \loss\big(f, X^{(i)}_z, Y^{(i)}_z \big),\;\forall z\in\mc{Z}$, with $\big(X^{(i)}_z, Y^{(i)}_z\big)_{i=1}^N$ being an \iid sequence of input-label pairs drawn from $P_z$.
% Here the subscript $z$ denotes the fact that $(X_z, Y_z)$  are drawn according to the distribution $P_z = P\lp \cdot , \cdot \mid Z=z\rp$.
\end{assumption}

The above assumption is a standard uniform convergence requirement which is satisfied by many commonly used families of classifiers. 
In the sequel, we will drop the $\mc{F}$ and $\delta$ dependence of $e_{z}(N, \mc{F}, \delta)$ and only refer to these terms as $e_{z}(N)$, for all $z \in \mc{Z}$ and $N \geq 1$. 

% \vspace{-0.5em}
% %----------------------------------------
% \subsection{Existence of Loss Equalizing Mixture Distribution}
% \label{subsec:existence}
% %===============================================================================
% \vspace{-0.5em}
% Before proceeding to the analysis of \algoref{algo:algo1}, we present a key result which states that under Assumptions~\ref{assump:ideal_case} and~\ref{assump:ideal_case2}, there exists a unique optimal mixture distribution $\pi^*$ that ensures the loss of all attributes, $\{L(z_i, f_{\pi^*})\}_{i=1}^m$, are equal. 

% \begin{proposition}
% \label{prop:sufficient}
% Suppose the conditional distributions $\{P_z : z \in \mc{Z} \}$, the loss function $\loss$, and the function class $\mc{F}$ satisfy Assumptions~\ref{assump:ideal_case} and~\ref{assump:ideal_case2}. Then, there exists a unique $\pi^* \in \Delta_m$ that achieves the optimal value for problem~\eqref{eq:optimal_mixture} and satisfies 
% %
% \begin{align*}
% \label{eq:pi_star1}
% L(z_1, f_{\pi^*}) = L(z_2, f_{\pi^*}) = \cdots = L(z_m, f_{\pi^*})\defined M^*.
% %   \mbb{E}_z \lb \loss(f_{\pi^*}, X, Y) \rb = \mbb{E}_{z'}\lb \loss(f_{\pi^*}, X, Y)\rb \defined M^*\qquad \forall \quad z, z' \in \mc{Z}.
% \end{align*}
% \end{proposition}
% %
% We report the proof of this proposition in Appendix~\ref{proof:proposition_sufficient}. 


% As mentioned earlier, there may exist problem instances where one of the groups is significantly \emph{easier} to classify than others, in which case Assumption~\ref{assump:ideal_case2}, and hence the conclusion of Proposition~\ref{prop:sufficient} does not hold. In those cases, it is reasonable to search for a Pareto optimal classifier with smallest minimax loss, as in \citep{martinez2020minimax}. We discuss this further in Sec.~\ref{sec:discussion}. 

% \mgh{Cannot you have the discussion about the relationship to Martinez here? If it doesn't need what you prove in the next sections, this might be a good place. Otherwise, write a line here and tell the reader about the discussion and refer to the Discussion section.}


%===============================================================================
%===============================================================================

% We now begin the analysis of our proposed adaptive sampling scheme, \algoref{algo:algo1}. Our first result, \propref{prop:consistency}, shows that our adaptive sampling scheme converges almost surely to an optimal mixture distribution $\pi^*$ as the sampling budget $n$ is taken to infinity. 

% \begin{proposition}
% \label{prop:consistency}
% Suppose Assumptions~\ref{assump:ideal_case},~\ref{assump:ideal_case2},~\ref{assump:ideal_case3} and~\ref{assump:uniform_deviation}
% % \assumpref{assump:ideal_case}, \assumpref{assump:ideal_case2}, \assumpref{assump:ideal_case3} and \assumpref{assump:uniform_deviation}
% hold. Then the mixture distribution, $\pi_n$, constructed by \algoref{algo:algo1} is asymptotically consistent. More formally, $\lim_{n \to \infty} \pi_n = \pi^*$ almost surely. 
% \end{proposition}

% \begin{proof}
% The proof follows from an application of Borel-Cantelli Lemma, and a modification of the statement of Lemma~\ref{lemma:forced_exploration}. \ssnotes{will add the details later.}
% \end{proof}

% Having established the asymptotic consistency of the mixture distribution generated by our algorithm, we now present a stronger result
\subsection{Analysis of Algorithm~\ref{algo:algo1}}
\label{subsec:analysis_algo1}
\vspace{-0.5em}
We now proceed to the analysis of our proposed optimistic adaptive sampling scheme ($\Aopt$) and state our main result, which is the convergence rate of the excess risk of $\Aopt$. %, in terms of the width of the uniform confidence sequence from \assumpref{assump:uniform_deviation}. 
Then in Remark~\ref{remark:instantiate}, we discuss how this general bound can be instantiated to obtain an explicit dependence on the budget $n$ for several important classifiers. 

\begin{theorem}
\label{theorem:regret_simple}
Let Assumptions~\ref{assump:ideal_case}-\ref{assump:uniform_deviation} hold and $\pi_{\min} \coloneqq \min_{z \in\mc{Z}}\pi^*(z)$. Fix any $A$ such that $\pi_{\min}/2 \leq A < \pi_{\min}$. Suppose   
% \begin{itemize}\itemsep0em
%     % \item \assumpref{assump:lipschitz} is satisfied~\ssnotes{most probably not needed},
%     \item \assumpref{assump:ideal_case}, \assumpref{assump:ideal_case2} and \assumpref{assump:ideal_case3} are satisfied by the distributions $\{ P_z: z \in \mc{Z}\}$, the function class $\mc{F}$ and the loss function $\loss$; and
%     \item \assumpref{assump:uniform_deviation} is satisfied by a sequence of terms $\{ e_{z}(N) \;:\; z \in \mc{Z}, N \geq 1\}$  with a given confidence level $\delta>0$; and
%     \item the query budget $n$ is sufficiently large, i.e., greater than a term $n_m$~(depending upon $A$ among other quantities) defined in \eqref{eq:ni}.
% \end{itemize}
the query budget $n$ is sufficiently large, as defined in Eq.~\ref{eq:ni} in Appendix~\ref{proof:excess_risk1}. Then, with probability $1-\delta$, the excess risk of \algoref{algo:algo1} can be upper-bounded as 

\vspace{-0.225in}
\begin{small}
\begin{equation}
\label{eq:excess-risk-Aopt}
\begin{split}
\mathcal{R}_n(\Aopt) &= \max_{z \in \mc{Z}} \; L(z, f_{\pi_n}) - M^* \\ 
&= \mc{O} \Big(\frac{ |\mc{Z}| C}{\pi_{\min}} \;\max_{z \in \mc{Z}} \; e_{z }(N_A)\Big),
\end{split}
\end{equation}
\end{small}
\vspace{-0.20in}

where $M^* = L(z, f_{\pi^*}),\;\forall z \in \mc{Z}$ (see Proposition~\ref{prop:sufficient}), $N_A = n \pi^2_{\min}/(2\pi_{\min}-A)$, and $C$ is the parameter introduced in Assumption~\ref{assump:ideal_case3}. 
\end{theorem}

% \mgh{Make sure this Eq. 19 in the statement of the Theorem does not change when you finalize the appendix.}

We provide a proof sketch for Theorem~\ref{theorem:regret_simple} at the end of this section and report its detailed proof in Appendix~\ref{proof:excess_risk1}. The result of Theorem~\ref{theorem:regret_simple} implies the following asymptotic rate of convergence for the expected excess risk of $\Aopt$. 

\begin{corollary}
\label{corollary:asymptotic}
Let the sequences $\big(e_z(N,\mc{F},\delta)\big)_{N\geq 1},\;\forall z\in\mc{Z}$, from~\assumpref{assump:uniform_deviation} satisfy the condition that  $\lim_{n \to \infty}e_z(\sqrt{n},\mc{F},1/n) = 0$. Then, by setting $\delta=1/n$ in Theorem~\ref{theorem:regret_simple}, we have 

\vspace{-0.20in}
\begin{small}
\begin{align*}
\label{eq:corollary1}
    \limsup_{n \to \infty} \; \frac{\mbb{E}\big[\mathcal{R}_n(\Aopt)\big]}{\max_{z \in \mc{Z}} \; e_z(N_A)} \; = \; \mc{O}\Big(\frac{|\mc{Z}| C}{\pi_{\min}}\Big). 
\end{align*}
\end{small}
\vspace{-0.20in}
\end{corollary}

Since the choice of $A < \pi_{\min}$ is arbitrary, $N_A$ can be made arbitrarily close to $n\pi_{\min}$. Thus, informally, the result of Corollary~\ref{corollary:asymptotic} indicates that the excess risk of $\Aopt$ converges to zero at the same rate as $ \max_{z \in \mc{Z}} e_z(n\pi_{\min})$. 


\begin{remark}
\label{remark:instantiate}
The bound on the excess risk of \algoref{algo:algo1} ($\Aopt$) derived in Theorem~\ref{theorem:regret_simple} (Eq.~\ref{eq:excess-risk-Aopt}) can be instantiated for several commonly used classifiers (function classes $\mathcal F$) to obtain an explicit convergence rate in $n$. If $\mc{F}$ has a finite VC dimension, $d_{VC}$, then we have $e_z(N) = \mc{O} \lp \nicefrac{d_{VC}}{ \sqrt{ N}}\rp$, which implies an asymptotic excess risk of $\mc{O} \lp \nicefrac{d_{VC}|\mc{Z}|C }{\pi^{1.5}_{\min}\sqrt{n} }\rp$ for $\Aopt$. If $\mc{F}$ has a Rademacher complexity of $\mc{O}\lp n^{-\alpha} \rp$, for some $\alpha>0$, then we obtain an excess risk bound of $\mc{O} \lp \nicefrac{|\mc{Z}|C}{\pi^{1+\alpha}_{\min} n^{\alpha}}\rp$ for $\Aopt$. These conditions on $\mathcal F$ are satisfied by several commonly used classifiers, such as linear, SVM, and multi-layer perceptron. 
\end{remark}

\begin{remark}[Knowledge of parameter $C$]
\label{remark:parameterC}
The implementation of \algoref{algo:algo1}, as described in Section~\ref{sec:algorithm}, requires the knowledge of the parameter $C$ (see Eq.~\ref{eq:ucb}) introduced in \assumpref{assump:ideal_case3}. This is primarily because we use the abstract expression $\{e_z(N): z \in \mc{Z},\;N \in \N\}$ in presenting and analyzing the algorithm. However, knowing $C$ is not strictly necessary to achieve the same asymptotic convergence rate as in Thm.~\ref{theorem:regret_simple} and Corollary~\ref{corollary:asymptotic}. For instance, if we know a constant $0<\zeta<1$, such that $1/e_z(N) = o(N^\zeta), \; \forall z \in \mc{Z}$, then we can achieve the same asymptotic excess risk rate by replacing $\sqrt{N_{z,t}}$ with $N_{z,t}^{\zeta}$  in Line~\ref{algoline:forced1} of \algoref{algo:algo1} and removing the $C$ dependent term from Line~\ref{algoline:choose1}. For most commonly used function classes $\mc{F}$, any choice of $\zeta>0.5$ should suffice. Further details are in Appendix~\ref{appendix:parameterC}.
\end{remark}

% \mgh{Fix this appendix.}

% \mgh{Here you are referring to Algorithm~1 and suddenly jump to Line 24 which is related to the longer version of Alg~1 in the appendix (Alg~2). This needs to be fixed. I'd suggest to refer to both Eq.~3 and the equation containing the exact value of $U$ on LIne 8 of Alg.~1.}

%===============================================================================

% \subsubsection{ Proof Outline of Theorem~\ref{theorem:regret_simple}.}

{\bf\em Proof Sketch of Theorem~\ref{theorem:regret_simple}.}
The proof proceeds in several `phases' (see Example~\ref{example:phases} in Appendix~\ref{proof:excess_risk1}) by partitioning the interval $[1,n]_\N$ into $[1, t_0]_\N, [t_0+1, t_1]_\N, \ldots, [t_{s-1}+1, t_s=n]_\N$, for some integer $0<s<|\mc{Z}|=m$. Here we use the notation $[u,v]_\N$ to represent $[u,v]\cap \N$. As we describe below, the end of each phase is marked by the last time an attribute from a certain non-empty subset of $\mc{Z}$ is sampled by the algorithm, and hence, the total number of phases, $s+1$, is smaller than $m$.  
% The high-level idea is as follows: suppose we have obtained an upper-bound on $\max_{z \in \mc{Z}} L(z, f_{\pi_{t_j}})$ for some $j \geq 0$. Then, we first identify those attributes whose proportion increased after time $t_j$, i.e., $z: \pi_{n}(z) > \pi_{t_j}(z)$, and define $t_{j+1}$ as the last time one such attribute is sampled. Denoting that attribute by $z_j$, we then employ the properties of our optimistic sampling rule (Line~\ref{algoline:choose1} of \algoref{algo:algo1}) to upper-bound the increase in $\max_{z} L(z, f_{\pi_{t_{j+1}}})$ during the phase~(we denote this term by $B_j$ which depends upon $\pi^*$ and $\lp e_z(N_{z, t_{j+1}}) \rp_{z \in \mc{Z}}$. Repeating this whole process $s$ times gives us the final result. 
% 
% 
% 
% \mgh{The last sentence of the above paragraph is too long and is hard to follow. How far the risk is?? Algorithm~1 has no Line~24, something is not right here. I think we should have an equation in the appendix that show this Line 24. We then say in the description of Alg.~1 that what really happens on Line~8 is that equation. Then, we can refer to that equation later, for example here. Finally, $L$ does not take $\pi$ as input. It takes $f_\pi$.}

We first note that unless $\pi_n = \pi^*$, in which case $\mc{R}_n(\Aopt)$ is zero, there must exist attributes $z$ for which $\pi_n(z) > \pi^*(z)$. We define $t_0$ as the last round that $\Aopt$ samples one such attribute and denote the corresponding attribute by $z_0$. Since $t_0<n$, we must have  $\pi_{t_0}(z_0) > \pi_n(z_0)> \pi^*(z_0)$, which due to the Assumption~\ref{assump:ideal_case} implies that $L(z_0, f_{\pi_{t_0}}) < L(z_0, f_{\pi^*}) = M^*$. Using this fact, we can show that $U_{t_0}(z_0, \hat{f}_{t_0}) \leq M^* + B_0$, where $B_0$ depends on $\big(e_{z}(N_{z,t_0})\big)_{z\in \mc{Z}}$ and $\pi^*(z_0)$ (see Lemma~\ref{lemma:over_represented} in Appendix~\ref{proof:excess_risk1}). Next, we observe that since $N_{z_0, t_0} > n\pi_{\min}$, for $n$ larger than $1/\pi_{\min}^2$, $z_0$ must have been selected at time $t_0$ due to the attribute selection rule in Line~\ref{algoline:choose1} of \algoref{algo:algo1}. We then use this to show 
% \mgh{When you refer to the selection rule, it refers to all those lines and not just Line~8, right? Do you wanna refer only to Line~8 or the whole thing?}
that $U_{t_0}(z, \hat{f}_{t_0}) \leq U_{t_0}(z_0, \hat{f}_{t_0})$ for all $z \neq z_0$, which implies that $L(z, f_{\pi_{t_0}}) \leq M^* + B_0$ for all $z \in \mc{Z}$. Thus, at the end of the first phase (i.e.,~at time $t_0$), the excess risk of $\Aopt$ is upper-bounded by $B_0$. 

Then, a technical result derived in Lemma~\ref{lemma:increase} (in Appendix~\ref{proof:excess_risk1}) ensures that there exists a non-empty subset $\Zover^{(1)}$ among the remaining attributes for which $\pi_{t_0}(z) < \pi_{n}(z),\;\forall z\in\Zover^{(1)}$. 
% These are attributes that are over-sampled (relative to $\pi_{t_0}$ in the interval $[t_0+1, n]_\N$). \mgh{I do not understand this sentence.}
% which follows from a   technical result stated in Lemma~\ref{lemma:increase}. 
We can then define $t_1$ as the last time an attribute from $\Zover^{(1)}$ is queried, and denote it by $z_1$. Similar to the previous case, we can then bound the value of $\max_{z \in \mc{Z}} L(z, f_{\pi_{t_1}})$ with $M^* + B_0 + B_1$, where $B_1$ depends on $\big(e_{z}(N_{z,t_1})\big)_{z \in \mc{Z}}$ and $\pi^*(z_1)$.
% \mgh{It only depends on the sequence or also $\pi^*(z_1)$, similar to the previous case?}
We repeat this process $s-1$ more times until the entire sampling budget is exhausted. The details of combining the above results to obtain the final statement of Theorem~\ref{theorem:regret_simple} are in Lemma~\ref{lemma:final_step} (Appendix~\ref{proof:excess_risk1}). 
% \mgh{Which details are in Lemma~5?}
\hfill \qedsymbol

% \end{proof}

%===============================================================================
% \subsubsection{Instantiating the Excess Risk}
% \label{sub2sec:instatiations}
% \ssnotes{remove this section}
%  In Theorem~\ref{theorem:regret_simple}, we have stated the excess risk upper bound in terms of the abstract terms $e_{z,N_{z,t}}$ introduced in \assumpref{assump:uniform_deviation}. By using existing uniform convergence results for commonly used function classes, we can instantiate the bound of Theorem~\ref{theorem:regret_simple} to make their dependence on $n$ explicit. 

% For the case of binary classification, if we assume that the loss function $\loss$ satisfies $|\loss(y, y')|\leq c_\loss$ for some $c_\loss <\infty$, then by using the Rademacher complexity based uniform deviation result \citep[Theorem~26.3]{shalev2014understanding},  we can set 
% \begin{align}
% &e_{z, N} = 2\mathfrak{R}_{N,z} + c_\loss \sqrt{\frac{2 \log \lp \nicefrac{2N^2}{3\delta} \rp}{N}}, \quad \text{where} \quad
%  \mathfrak{R}_{N,z} \coloneqq  \mbb{E}_{S_N \sim P_z^{\otimes N}}\; \mbb{E}_\sigma \lb \sup_{f \in \mc{F}} \frac{1}{N} \sum_{(x,y) \in S_N} \sigma_i \loss\lp f, x, y \rp \rb
% \end{align}
% to ensure that \assumpref{assump:uniform_deviation} is satisfied. In the above display, $\sigma_i \sim \text{Uniform}\lp \{+1, -1\} \rp$ for $1 \leq i \leq N$ are \iid Rademacher random variables, and $\mathfrak{R}_{N,z}$
% is used to denote the Rademacher complexity associated with $(\mc{F}, \loss, P_z)$ triplet.  We can now apply this result to derive explicit bounds on the excess risk for some commonly used function classes. 
% %----------------------------------------


%  \tbf{Linear classifiers and SVMs.} Suppose $\mc{X} = [-B, B]^d \subset \mathbb{R}^d$, $\mc{F} = \{\langle x, w \rangle : \|w\|_2 \leq 1 \}$, and the loss function   $\loss:\reals\times \reals \mapsto [0,\infty)$ is $1-$Lipschitz. Note that here we are assume a special case of  $\loss(f, x, y) = \loss(f(x), y)$. Then  by a minor modification of the proof of \citep[Lemma~26.10]{shalev2014understanding}, we can show that for  this case we have $\mathfrak{R}_{N,z} \leq \nicefrac{\mbb{E}_z \lb \|X\|_2\rb}{\sqrt{N}}$, which implies that 
%  \begin{align}
%  \max_{z \in \mc{Z}} \Ez{f_{\pi_n}} - M^* &= \mc{O} \lp  \frac{|\mc{Z}|C}{a} \;\; \frac{ B + c_\loss \sqrt{4\log\lp \nicefrac{a^2n^2\pi^2}{12\delta}\rp}}  {\sqrt{a n}}  \rp.
%  \end{align}
 
% The above derived excess-risk bound for the case of linear classifiers can be used to obtain similar bounds for the case of the constrained versions of SVM. 

% %----------------------------------------
% \tbf{Neural Networks.} For small feedforward neural networks, we can use the existing bounds on the VC dimension~($d_{VC}$), such as \citep[Lemma~20.14]{shalev2014understanding}, which say that $d_{VC} = \mc{O} \lp m_E\log m_E \rp$ for a class of neural networks represented by a computational graph with $m_E$ edges. Plugging this into the statement of Theorem~\ref{theorem:regret_simple} gives us 
%  \begin{align}
%  \max_{z \in \mc{Z}} \Ez{f_{\pi_n}} - M^* &= \mc{O} \lp  \frac{|\mc{Z}|C}{a} \;\; \frac{ \sqrt{m_E \log m_E} + c_\loss \sqrt{4\log\lp \nicefrac{a^2n^2\pi^2}{12\delta}\rp}}  {\sqrt{ a n}}  \rp.
%  \end{align}
 
% However, these bounds turn out to be vacuous in the case of modern overparameterized networks, and in those cases other unifrom deviation bounds such as the norm-based bounds derived in \citep{neyshabur2015norm} may be used. 


% %================================================================================

%===============================================================================
%===============================================================================

%===============================================================================
% LOwer Bounds
%===============================================================================

\subsection{Lower Bound}
\label{subsec:lower_bound}

\vspace{-0.5em}
We first introduce some notation for presenting our lower-bound results. We denote by $\mc{M}$ the class of $\toymodel$s introduced in Definition~\ref{def:toymodel}. We also define the following class of problems:

\begin{definition}
\label{def:Q}
We use $\mc{Q}$ to denote the class of problems defined by the triplets $(\bm{\mu}, \mc{F}, \loss_{01})$, where $\bm{\mu} \in \mc{M}$ is an instance of the \toymodel, $\mc{F}$ is the class of linear classifiers in two dimensions, and $\loss_{01}$ is the $0-1$ loss. 
\end{definition}

For the function class $\mc{F}$, we know that $e_{z}(N) = \mc{O} ( 1/\sqrt{N})$ for both $z \in \mc{Z} = \{u, v\}$, which implies that the excess risk achieved by both $\Aopt$ and \epsg strategies is of $\mc{O}\lp 1/\sqrt{n} \rp$. We now prove (in Appendix~\ref{appendix:proof_lower}) that this convergence rate (in terms of $n$) cannot in general be improved. 

\begin{proposition}
\label{prop:lower} 
Suppose $\mc{A}$ is any adaptive sampling scheme which is applied with a budget $n$ to a problem $Q \in \mc{Q}$ introduced in Definition~\ref{def:Q}. Then, we have 

\vspace{-0.2in}
\begin{small}
\begin{align}
    \max_{Q \in \mc{Q}}\; \mbb{E}_Q\lb \mc{R}_n \lp \mc{A} \rp  \rb = \Omega \lp 1/\sqrt{n} \rp. 
\end{align}
\end{small}
\vspace{-0.2in}
\end{proposition}

\vspace{-1em}
